Experimenting with Normalization Layers in Federated Learning on non-IID scenarios

Training Deep Learning (DL) models require large, high-quality datasets, often assembled with data from different institutions. Federated Learning (FL) has been emerging as a method for privacy-preserving pooling of datasets employing collaborative training from different institutions by iteratively globally aggregating locally trained models. One critical performance challenge of FL is operating on datasets not independently and identically distributed (non-IID) among the federation participants. Even though this fragility cannot be eliminated, it can be debunked by a suitable optimization of two hyper-parameters: layer normalization methods and collaboration frequency selection. In this work, we benchmark five different normalization layers for training Neural Networks (NNs), two families of non-IID data skew, and two datasets. Results show that Batch Normalization, widely employed for centralized DL, is not the best choice for FL, whereas Group and Layer Normalization consistently outperform Batch Normalization. Similarly, frequent model aggregation decreases convergence speed and mode quality.

==> 8. TNNLS - EXPERIMENTING WITH NORMALIZATION LAYERS IN FL/.git/objects/1c/2fa8119e3fdc2a52985499cd57b4bae87b60f2 <==
xŽMjÄ0F»ö)´/'ÿä@)¥=‰"ËíÐdR‡¹þzƒÙ}¼Å{ŸnëzàCzÝØRãÊ­Rm¤Á[±â'Ç0•4çÈ…=¹?évYšf"•‰¨¦Âq.[Ž!Öª©"ª4«"cül>ûqÛàKv[7ýÈSùø^åº\t[߁ò™ˆHLðŠ"èNzÞö´ÀÝM~¡Û~,cwô¡I

==> 8. TNNLS - EXPERIMENTING WITH NORMALIZATION LAYERS IN FL/.git/objects/58/0ea1ed9783255e424155498d48a2e3e5f003a7 <==
xŽ[
Â0EýÎ*æ_$Î$ "º'iZhIÓý[pþ]΁Ã
µ"¹ƒèÔ[J0&"QGöYxÖàd):3ù0u¶ÔGZZ;0£wȖ)f&"o"¦ÉxŒ>;""'½¿kƒGÛ×
OÙÒ²\Ãohöîþ*2/—PË
1Z$ËÎÚh­zÜìéï€*ë¼uhiۗ¾©/)Is

==> 8. TNNLS - EXPERIMENTING WITH NORMALIZATION LAYERS IN FL/.git/objects/6b/678802ad7aa8dd2d5bf17a91c48769879df726 <==
xOKNÃ0eSÌ®"`Çv'F!PHÐ
\`<¶S‹$®Œ{\!.Àîé}õ8¯kª Œ¹©%ÀÑ+éå^XcÔz•Qˆ'½F‡l}0jÏݙJØ*	4¬QZË{"ŒV;%xB‹Fû@WM4õϯI'i!
!
i£›¦è+Í£³ž¥ñ24®£K=åÏå²ex¡ï°,üÚéi^)-çõd›FaôhàVH!ºÆ¶[5ü» {eà
m|']›Úv#Ì©.䟆˖jR½§å|¢»qì_‡Cÿy<¾}ô.´ØJ嫏¤­f¸6t?l=o

==> 8. TNNLS - EXPERIMENTING WITH NORMALIZATION LAYERS IN FL/.git/objects/74/0140c86ace4fb6fed126662e27445db478d56c <==
xŽKjÄ0³Ö)zÔn}lœ¤Õj;Ë
ùþcÈ
fW<¨GI«µ˜\ø]0;&\'c¯³$"ì'ϙ2YZYyñ!Sœ'óÇ]'e
¢"a]WM)ÛÀÑrpY¬X\"qR2|ŽßÖởGƒ~ê¾3Üål\æÇV¹ì7iõ0Dr#ø´h­¹Ö+sèÛæÜ/»´^€·­œÏÁõê/æF2O

==> 8. TNNLS - EXPERIMENTING WITH NORMALIZATION LAYERS IN FL/.git/objects/8c/20b57dec31e0de1e0ed3fda57382fafe47610f <==
xÎA
Â0…a×9Å왉é$ѓL§S-´M‰ñþ¼»Ç¿x|Z–ejàZ5ò>§"9¢dÉÆ]ŠQ•…óЋŽ"¢Û¤ÚÚ 'FCÏ^e£'œ-°‰Ð§ûØQïäÓ^¥Â½~ÖyÛ<\ô70æt{.2Í'-ˈã™=êàˆ"èöº3›ý}àtžvïv·<«l/÷}YK2

==> 8. TNNLS - EXPERIMENTING WITH NORMALIZATION LAYERS IN FL/.git/objects/a0/0eacb96e672716a11bed9d12e346c2e5f424a1 <==
xŽ]
Â0"}Î)ö]Ý4͈ˆžd"nk¡i%Mñú¼oÃßǤ-繂6þT‹Dêp`ñVvÉ%
.JÀD4ZÖ¨û¤YD½¹ÈZA(ȶ1bH»`}ÄÎS¡R›z3Žlõµx"cÝàÉ»,Ã5ýºàïSæy¹¤-߀¬ëÉYç&AÕÚv³Êß5ÎÓQd‡Ï\_…Wàu€½êÑMÎ

==> 8. TNNLS - EXPERIMENTING WITH NORMALIZATION LAYERS IN FL/.git/objects/b0/50bb884fafc9f34629ccb40d3a2147131b36f5 <==
x]j1ƒûœSø}¡Øq&?°"²=‰›8m`2S²™û7ÐôE|$¤|öÞ&Ø;̡
)aNe#F¯Á'¸B\]t¬QÙƒÄ%ÏæG†b¶ø¹…¢™I±è-\‹l£­RÕOX\óûð×q‡<ußîù0¤øþÕ¥í¯ùìo@~¥=3¸!!šå®™Sÿ]`®}¶Þ`´ç"™
´Ö–Ûúpè4¿†P

==> 8. TNNLS - EXPERIMENTING WITH NORMALIZATION LAYERS IN FL/.git/objects/ba/79c91300318276aaa311a4ff8449d5a215f911 <==
xŽM
Â0F]ç³dòÓLDDéBðÓt¢Bk¥¦àñ-x7·x|yÇGçý¦ÎªÐ¤d…É%҂¾8v¡WvQQ…cAŠXÌKf}VàK¹Ä¾'ìŠ×Ðqc³&D^·'jØgjŒ,õ>Ípš—çgyë0ìó8o£<†]žÆØÉ3Ùà`‹Ѭv½YõJÕ\Ú¶5_ÛG±

==> 8. TNNLS - EXPERIMENTING WITH NORMALIZATION LAYERS IN FL/.git/objects/c9/17bd08eb123c5413c2b02f2306942201e33493 <==
xŽA
Â0E]çً'IÒt
"¢'™L¦*$M‰éý-xwŸïñ¹–òîÚ:8ô&¢"ˆ"ÎÛgà™R°È1Åaƀdi"¨Vj²thM`&wØNÀä9¤èÝìه)Š‹³¢­¿jÓ÷¶-U?è#9"¾ðo˜qÂÛ³Ð;Ÿ¹–«†0Bp0ºQ
£vºßìòw@­MN떳ú\¶I"

==> 8. TNNLS - EXPERIMENTING WITH NORMALIZATION LAYERS IN FL/.git/objects/f2/73c29a84bb366f5999688ffc9805ed2215c0ad <==
x¥ÎAj!…á¬=EíƒekiòIhYM\LÛh5ÌñgHrƒìßâñs¿Ýš'#zÑ!eubm6yb‡±¢O9²IÉqc—À±š#ÙRr–˜³-"Ù­ÈÙ3Õâ—ͳ§µÈR6"Oýî¾z'¡>æÑg{Žëø•‹üÉû¹?ýÒô
"ŸhExµh­áŸZ•ÿþ˜Ïv—
óÈ,òèç^›fm}ŸæÚgXº

==> 8. TNNLS - EXPERIMENTING WITH NORMALIZATION LAYERS IN FL/.git/objects/f3/d0986924a6a50b1d77398536d89077bb4ce003 <==
x­ŽAjÃ0E»Ö)´/ld¥=@1'F
B.>~Ms…¬Þß¼Ïãv¿ë°ÝÛè"ó…0g\.Íe… @	üÆ)¬S"\Ä<¨K=ńEHVZÃÆnƒYRæeFñ1$p`Žœ©ÚÇ­uûM›ýúÉZwfµzÎÏ_íW­JSևÖÒNN{ÕÑ&0"ˆñÌ´ïœ3üß=äuæ8ó#!U¢
